Fractal Dimension of Self-Affine Signals: Four Methods of Estimation

This paper serves as a complementary material to a poster presented at the XXXVI Dynamics Days Europe in Corfu, Greece, on June 6th-10th in 2016. In this study, fractal dimension ($D$) of two types of self-affine signals were estimated with help of four methods of fractal complexity analysis. The methods include the Higuchi method for the fractal dimension computation, the estimation of the spectral decay ($\beta$), the generalized Hurst exponent ($H$), and the detrended fluctuation analysis. For self-affine processes, the next relation between the fractal dimension, Hurst exponent, and spectral decay is valid: $D=2-H=\frac{5-\beta}{2}$. Therefore, the fractal dimension can be get from any of the listed characteristics. The goal of the study is to find out which of the four methods is the most reliable. For this purpose, two types of test data with exactly given fractal dimensions ($D = 1.2, 1.4, 1.5, 1.6, 1.8$) were generated: the graph of the self-affine Weierstrass function and the statistically self-affine fractional Brownian motion. The four methods were tested on the both types of time series. Effect of noise added to data and effect of the length of the data were also investigated. The most biased results were obtained by the spectral method. The Higuchi method and the generalized Hurst exponent were the most successful.

==> referencesm.tex <==
% This file was created with JabRef 2.8.1.
% Encoding: Cp1250

@book{falco2004,
  title={Fractal geometry: mathematical foundations and applications},
  author={Falconer, Kenneth},
  year={2004},
  publisher={John Wiley \& Sons}
}

@ARTICLE{abry1996,
  author = {Abry, Patrice and Sellan, Fabrice},
  title = {The wavelet-based synthesis for fractional Brownian motion proposed
	by F. Sellan and Y. Meyer: Remarks and fast implementation},
  journal = {Applied and computational harmonic analysis},
  year = {1996},
  volume = {3},
  pages = {377--383},
  number = {4},
  publisher = {Elsevier}
}

@book{mande1983,
  title={The fractal geometry of nature},
  author={Mandelbrot, Benoit B},
  volume={173},
  year={1983},
  publisher={Macmillan}
}

@ARTICLE{Axelsson,
  author = {O. Axelsson},
  title = {Conjugate gradient type methods for unsymmetric and inconsistent
	systems of linear equations},
  journal = {Linear Algebra Appl.},
  year = {1980},
  volume = {29},
  pages = {1-16}
}

@ARTICLE{Brown-Saad1,
  author = {P. N. Brown and Y. Saad},
  title = {Hybrid {K}rylov methods for nonlinear systems of equations},
  journal = {SIAM J. Sci. Statist. Comput.},
  year = {1990},
  volume = {11},
  pages = {450-481}
}

@INPROCEEDINGS{bs,
  author = {R. A. Brualdi and B. L. Shader},
  title = {On sign-nonsingular matrices and the conversion of the permanent
	into the determinant},
  booktitle = {Applied Geometry and Discrete Mathematics},
  year = {1991},
  editor = {P. Gritzmann and B. Sturmfels},
  pages = {117-134},
  address = {Providence, RI},
  publisher = {American Mathematical Society}
}

@ARTICLE{DES,
  author = {R. S. Dembo and S. C. Eisenstat and T. Steihaug},
  title = {Inexact {N}ewton methods},
  journal = {SIAM J. Numer. Anal.},
  year = {1982},
  volume = {19},
  pages = {400-408}
}

@ARTICLE{djd,
  author = {J. Drew and C. R. Johnson and P. {van den Driessche}},
  title = {Strong forms of nonsingularity},
  journal = {Linear Algebra Appl.},
  year = {1992},
  volume = {162},
  note = {to appear}
}

@ARTICLE{EES,
  author = {S. C. Eisenstat and H. C. Elman and M. H. Schultz},
  title = {Variational iterative methods for nonsymmetric systems of linear
	equations},
  journal = {SIAM J. Numer. Anal.},
  year = {1983},
  volume = {20},
  pages = {345-357}
}

@PHDTHESIS{Elman,
  author = {H. C. Elman},
  title = {Iterative methods for large, sparse, nonsymmetric systems of linear
	equations},
  school = {Department of Computer Science, Yale University, New Haven, CT},
  year = {1982}
}

@ARTICLE{g,
  author = {P. M. Gibson},
  title = {Conversion of the permanent into the determinant},
  journal = {Proc. Amer. Math. Soc.},
  year = {1971},
  volume = {27},
  pages = {471-476}
}

@ARTICLE{GloKR85,
  author = {R. Glowinski and H. B. Keller and L. Rheinhart},
  title = {Continuation-conjugate gradient methods for the least-squares solution
	of nonlinear boundary value problems},
  journal = {SIAM J. Sci. Statist. Comput.},
  year = {1985},
  volume = {6},
  pages = {793-832}
}

@BOOK{Golub-VanLoan,
  title = {Matrix Computations, Second ed.},
  publisher = {The Johns Hopkins University Press},
  year = {1989},
  author = {G. H. Golub and C. F. {Van Loan}},
  address = {Baltimore, MD}
}

@ARTICLE{klm,
  author = {V. Klee and R. Ladner and R. Manber},
  title = {Signsolvability revisited},
  journal = {Linear Algebra Appl.},
  year = {1984},
  volume = {59},
  pages = {131-157}
}

@INPROCEEDINGS{More,
  author = {J. J. Mor\'e},
  title = {A collection of nonlinear model problems},
  booktitle = {Computational Solutions of Nonlinear Systems of Equations},
  year = {1990},
  editor = {E. L. Allgower and K. Georg},
  volume = {26},
  series = {Lectures in Applied Mathematics},
  pages = {723-762},
  address = {Providence, RI},
  publisher = {American Mathematical Society}
}

@ARTICLE{m,
  author = {K. Murota},
  title = {{LU} decomposition of a matrix with entries of different kinds},
  journal = {Linear Algebra Appl.},
  year = {1983},
  volume = {49},
  pages = {275--283}
}

@ARTICLE{Saad,
  author = {Y. Saad},
  title = {Krylov subspace methods for solving large unsymmetric linear systems},
  journal = {Math. Comp.},
  year = {1981},
  volume = {37},
  pages = {105-126}
}

@ARTICLE{Saad-Schultz,
  author = {Y. Saad and M. H. Schultz},
  title = {{GMRES}: A generalized minimal residual method for solving nonsymmetric
	linear systems},
  journal = {SIAM J. Sci. Statist. Comput.},
  year = {1986},
  volume = {7},
  pages = {856-869}
}

@ARTICLE{Swarztrauber-Sweet,
  author = {P. N. Swarztrauber and R. A. Sweet},
  title = {Efficient {FORTRAN} subprograms for the solution of elliptic partial
	differential equations},
  journal = {ACM Trans. Math. Software},
  year = {1979},
  volume = {5},
  pages = {352-364}
}

@ARTICLE{Walker89,
  author = {H. F. Walker},
  title = {Implementations of the {GMRES} method},
  journal = {Computer Phys. Comm.},
  year = {1989},
  volume = {53},
  pages = {311-320}
}

@ARTICLE{Walker88,
  author = {H. F. Walker},
  title = {Implementation of the {GMRES} method using {H}ouseholder transformations},
  journal = {SIAM J. Sci. Statist. Comput.},
  year = {1988},
  volume = {9},
  pages = {152-163}
}

@Book{abarb1996,
  AUTHOR = 	"Abarbanel, H. D. I.",
  TITLE = 	"Analysis of Observed Chaotic Data",
  YEAR = 	"1996",
  PUBLISHER = 	"Springer"}

@Article{acher1998,
    AUTHOR = 	"Achermann, P. and Borb\'{e}ly, A. A.",
    TITLE = 	"Coherence analysis of the human sleep electroencephalogram",
    YEAR = 	"1998",
    JOURNAL = 	"Neuroscience",
    VOLUME = 	"85",
    PAGES = 	"1195-1208"}

@Article{acher1998b,
    AUTHOR = 	"Achermann, P. and Borb\'{e}ly, A. A.",
    TITLE = 	"Temporal evolution of coherence and power in the human sleep electroencephalogram",
    YEAR = 	"1998",
    JOURNAL = 	"J Sleep Res ",
    VOLUME = 	"7",
    ISSUE =  "S1",
    PAGES = 	"36-41"}


@Article{acher2003,
  AUTHOR = 	"Achermann, P. and Borb\'{e}ly, A. A.",
  TITLE = 	"Mathematical Models of Sleep Regulation.",
  YEAR = 	"2003",
  JOURNAL = 	"Frontiers in Bioscience",
  VOLUME = 	"8",
  PAGES = 	"683-693"}  

@Article{aftan1997,
    AUTHOR = 	"Aftanas, L. I. and others",
    TITLE = 	"Nonlinear Forecasting Measurements of the Human {EEG} During Evoked Emotions",
    YEAR = 	"1997",
    JOURNAL = 	"Brain Topography",
    VOLUME = 	"10",
    PAGES = 	"155-162"}

@Article{aftan2002,
    AUTHOR = 	"Aftanas, L. and Golocheikine, S.	",
    TITLE = 	"Non-linear dynamic complexity of the human {EEG} during meditation",
    YEAR = 	"2002",
    JOURNAL = 	"Neurosci Lett",
    VOLUME = 	"330",
    PAGES = 	"143-146"}
  
@Article{aguir2008,
    AUTHOR = "Aguirre, L. A. and Bastos, S. B. and Alves, M. A. and Letellier C.",
    TITLE = "Observability of nonlinear dynamics: Normalized results and a time-series approach",
    YEAR = "2008",
    JOURNAL = "Chaos",
    VOLUME = "18",
     PAGES = " 013123"}

@Article{aguir2011,
    AUTHOR = "Aguirre, L. A. and Letellier C.",
    TITLE = "Investigating observability properties from data in nonlinear dynamics",
    YEAR = "2011",
    JOURNAL = "Physical Review E",
    VOLUME = "83",
     PAGES = "066209"}

@Article{ander2005,
  AUTHOR = 	"Anderer, P. and Gruber, G. and Parapatics, S. and Woertz, M. and Miazhynskaia, T. and Kl{\"o}sch, G. and Saletu, B. and Zeitlhofer, J. and Barbanoj, M., J. and Danker-Hopfe, H. and Himanen, S.-L. and Kemp, B. and Penzel, T. and Gr{\"o}zinger, M. and Kunz, D. and Rappelsberger, P. and Schl{\"o}gl, A. and Dorffner, G.",
  TITLE =	"An {E}-{H}ealth {S}olution for {A}utomatic {S}leep {C}lassification according to {R}echtschaffen and {K}ales: {V}alidation {S}tudy of the {S}omnolyzer 24 x 7 {U}tilizing the {S}iesta {D}atabase",
  JOURNAL =	"Neuropsychobiology",
  VOLUME =	"51",
  NUMBER = "3",
  YEAR =	"2005",
  PAGES =	"115-133"}

@Article{andre1996,
  AUTHOR = 	"Andrew, C. and Pfurtscheller, G.",
  TITLE =	"Event-related coherence as a tool for studying dynamic interaction of brain regions ",
  JOURNAL =	"Electroencephalogr Clin Neurophysiol ",
  VOLUME =	"98",
  NUMBER = "2",
  YEAR =	"1996",
  PAGES =	"144-148"}

@Article{andrz2001,
    AUTHOR = 	"Andrzejak, Ralph G and others",
    TITLE = 	"Indications of nonlinear deterministic and  finite-dimensional structures in time series     of 
    brain electrical activity: Dependence on recording region and brain state	",
    YEAR = 	"2001",
    JOURNAL = 	"Phys. Rev. Letters",
    VOLUME = 	"64, 061907",
    PAGES = 	"1-8"}

@article{andrz2003,
  title={Bivariate surrogate techniques: necessity, strengths, and caveats},
  author={Andrzejak, Ralph G and Kraskov, Alexander and St{\"o}gbauer, Harald and Mormann, Florian and Kreuz, Thomas},
  journal={Physical review E},
  volume={68},
  number={6},
  pages={066202},
  year={2003},
  publisher={APS}
}

@article{andrz2011,
  title={Characterizing unidirectional couplings between point processes and flows},
  author={Andrzejak, Ralph G and Kreuz, Thomas},
  journal={EPL (Europhysics Letters)},
  volume={96},
  number={5},
  pages={50012},
  year={2011},
  publisher={IOP Publishing}
}  

@Article{angel2004,
  title = {Steady-State Visual Evoked Potentials and Phase Synchronization in Migraine Patients},
  author = {Angelini, L.  and Tommaso, M. De and Guido, M.  and Hu, K.  and Ivanov, P. Ch. and Marinazzo, D.  and Nardulli, G.  and Nitti, L.  and Pellicoro, M.  and Pierro, C.  and Stramaglia, S. },
  journal = {Phys Rev Lett},
  volume = {93},
  number = {3},
  pages = {038103},
  numpages = {4},
  year = {2004},
}

@article{arnho1999,
  title={A robust method for detecting interdependences: application to intracranially recorded EEG},
  author={Arnhold, Jochen and Grassberger, Peter and Lehnertz, Klaus and Elger, Christian Erich},
  journal={Physica D: Nonlinear Phenomena},
  volume={134},
  number={4},
  pages={419--430},
  year={1999},
  publisher={Elsevier}
}  

@Article{aseri1953,
  AUTHOR = 	"Aserinsky, E. and Kleitman, N.	",
  TITLE = 	"Regularly {O}ccurring {P}eriods of {E}ye {M}otility, and {C}oncomitant {P}henomena, {D}uring {S}leep",
  YEAR = 	"1953",
  JOURNAL = 	"Science",
  VOLUME = 	"118",
  PAGES = 	"273-274"}

@Book{atwoo1989,
  AUTHOR = 	"Atwood, H. L. and MacKay, W. A.",
  TITLE = 	"Essentials of Neurophysiology",
  YEAR = 	"1989",
  PUBLISHER = 	"B.C. Decker Inc"}

@Article{bablo1985,
  AUTHOR = 	"Babloyantz, A. and Salazar, J. M. and Nicolis C.",
  TITLE = 	"Evidence of chaotic dynamics of brain activity during the sleep cycle",
  YEAR = 	"1985",
  JOURNAL = 	"Physics Letters A",
  VOLUME = 	"111",
  NUMBER = "3",
  PAGES = 	"152-156"}

@Article{bak1987,
	AUTHOR = "Bak, P. and Tang, C. and Wiesenfeld, K.",
	TITLE = "Self-organized criticality: {A}n explanation of 1/f noise.",	
	JOURNAL = "Phys Rev Lett",
	VOLUME = "59",
	NUMBER = "4",
	YEAR = "1987",
	PAGES = "381-384"
}
  
@Article{bankm1992,
  AUTHOR = 	"Bankman, I. N. and Sigillito, V. G. and Wise, R. A. and Smith, P. L.",
  TITLE = 	"Feature-based detection of the {K}-complex wave in the human electroencephalogram using neural networks",
  YEAR = 	"1992",
  JOURNAL = 	"IEEE Transactions on Biomedical Engineering",
  VOLUME = 	"39(12)",
  PAGES = 	"1305-1310"}

@article{barne2009,
  title={Granger causality and transfer entropy are equivalent for Gaussian variables},
  author={Barnett, Lionel and Barrett, Adam B and Seth, Anil K},
  journal={Physical review letters},
  volume={103},
  number={23},
  pages={238701},
  year={2009},
  publisher={APS}
}

@Article{bhatt2001,
	AUTHOR = "Bhattacharya, J. and Petsche, .H. and Feldmann, U. and Rescher, B.",
	TITLE = "{EEG} gamma-band phase synchronization between posterior and frontal cortex during mental rotation in humans",	
	JOURNAL = "Neurosci Lett",
	VOLUME = "311",
	NUMBER = "1",
	YEAR = "2001",
	PAGES = "29-32"
}

@Article{bob2008,
	AUTHOR = "Bob, P. and Palu\v{s}, M. and \v{S}usta, M. and Glaslov\'{a}, K.",
	TITLE = "{EEG} phase synchronization in patients with paranoid schizophrenia",	
	JOURNAL = "Neurosci Lett",
	VOLUME = "447",
	NUMBER = "1",
	YEAR = "2008",
	PAGES = "73 - 77"
}
  
@Article{borbe1981,
  AUTHOR = 	"Borb\'{e}ly, A. A. and Baumann, F. and  Brandeis, D. and Strauch, I. and Lehmann, D.",
  TITLE = 	"Sleep Deprivation: Effect on Sleep Stages and {EEG} Power Density in Man.",
  YEAR = 	"1981",
  JOURNAL = 	"Electroencephalogr Clin Neurophysiol ",
  NUMBER = "5",
  VOLUME = 	"51",
  PAGES = 	"483-493"}
 
@Article{brand2000,
    AUTHOR = "Brandt, M. E. and Ademo\v{g}lu, A. and Pritchard, W. S	",
    TITLE = "Nonlinear Prediction and Complexity of Alpha {EEG} Activity",
    YEAR = "2000",
    JOURNAL = "International Journal of Bifurcation and Chaos",
    VOLUME = "10",
    NUMBER = "1",
    PAGES = "123-133"}

@Article{brazi1949,
    AUTHOR = "Brazier, M. A. B.",
    TITLE = "A study of the electrical field at the surface of the head",
    YEAR = "1949",
    JOURNAL = "Electroencephalogr Clin Neurophysiol ",
    VOLUME = "1",
    NUMBER = "1-4", 
    PAGES = "195-204"}

@Article{broug1995,
    AUTHOR = "Broughton, R. and Hasan, J.",
    TITLE = "Quantitative topographic electroencephalographic mapping during drowsiness and sleep onset",
    YEAR = "1995",
    JOURNAL = "J Clin Neurophysiol",
    VOLUME = "12(4)",
    PAGES = "372-386"}

@article{brown2012,
  title={Conditional likelihood maximisation: a unifying framework for information theoretic feature selection},
  author={Brown, Gavin and Pocock, Adam and Zhao, Ming-Jie and Luj{\'a}n, Mikel},
  journal={The Journal of Machine Learning Research},
  volume={13},
  number={1},
  pages={27--66},
  year={2012},
  publisher={JMLR. org}
}

@Article{buchs1982,
    AUTHOR = "Buchsbaum, M. S. and Mendelson, W. B. and Duncan, W. C. and Coppola, R. and Kelsoe, J. and Gillin, J. C.",
    TITLE = "Topographic cortical mapping of {EEG} sleep stages during daytime naps in normal subjects",
    YEAR = "1982",
    JOURNAL = "Sleep",
    VOLUME = "5",
    NUMBER = "3",
    PAGES = "248-255"}

@Article{cai1991,
    AUTHOR = 	"Cai, Z.-J.",
    TITLE = 	"The Function of Sleep: Further Analysis",
    YEAR = 	"1991",
    JOURNAL = 	"Physiology \& Behavior",
    NUMBER = "1",
    VOLUME = 	"50",
    PAGES = 	"53-60"}

@Article{cajoc1995,
  AUTHOR = 	"Cajochen, C. and Brunner, D. P. and Kr?uchi, K. and Graw, P. and Wirz-Justice, A.",
  TITLE = 	"Power density in theta/alpha frequencies of the waking {EEG} progressively increases during sustained wakefulness",
  YEAR = 	"1995",
  JOURNAL = 	"Sleep",
  VOLUME = 	"18",
  NUMBER = "10",
  PAGES = 	"890-894"}
  
@Article{cajoc2003,
  AUTHOR = 	"Cajochen, C. and Dijk, D. J.",
  TITLE = 	"Electroencephalographic activity during wakefulness, rapid eye movement and non-rapid eye    
  movement sleep in humans: Comparison of their circadian and homeostatic modulation",
  YEAR = 	"2003",
  JOURNAL = 	"Sleep and Biological Rhythms",
  VOLUME = 	"1",
  NUMBER = "2",
  PAGES = 	"85-95"}
  
@Article{campa2004,
  AUTHOR = 	"Campagne, A. and Pebayle, T. and Muzet, A.",
  TITLE = 	"Correlation between driving errors and vigilance level: influence of the driver?s age",
  YEAR = 	"2004",
  JOURNAL = 	"Physiology and Behavior",
  VOLUME = 	"80",
  PAGES = 	"515?524"}
 
@Article{cante1999,
  AUTHOR = 	"Cantero, J. L. and Atienza, M. and Salas, R. M. and G{\'o}mez, C. M.",
  TITLE = 	"Alpha {EEG} coherence in different brain states: an electrophysiological index of the arousal level in human subjects",
  YEAR = 	"1999",
  JOURNAL = 	"Neurosci Lett",
  VOLUME = 	"271",
  NUMBER = "3",
  PAGES = 	"167-170"} 
    
@Article{cante2002,
  AUTHOR = 	"Cantero, J. L. and Atienza, M. and Salas, R. M.",
  TITLE = 	"Human alpha oscillations in wakefulness, drowsiness period, and {REM} sleep: different electroencephalographic phenomena within the alpha band",
  YEAR = 	"2002",
  JOURNAL = 	"Clin Neurophysiol",
  VOLUME = 	"32",
  NUMBER = "1",
  PAGES = 	"54-71"}
  
@Article{cante2004,
  AUTHOR = 	"Cantero, J. L. and Atienza, M. and Madsen, J. R. and Stickgold, R.",
  TITLE = 	"Gamma {EEG} dynamics in neocortex and hippocampus during human wakefulness and sleep",
  YEAR = 	"2004",
  JOURNAL = 	"NeuroImage",
  VOLUME = 	"22(3)",
  NUMBER = "3",
  PAGES = 	"1271-1280"}

@Article{cao1997	,
	AUTHOR = "Cao, L.",
	TITLE = "Practical method for determining the minimum embedding dimension of a scalar time series",	
	JOURNAL = "Physica D",
	VOLUME = "110",
	NUMBER = " ",
	YEAR = "1997",
	PAGES = "43-50"
}
 	 
@Article{casda1989,
    AUTHOR = 	"Casdagli, M.	",
    TITLE = 	"Nonlinear Prediction of Chaotic Time Series",
    YEAR = 	"1989",
    JOURNAL = 	"Physica D",
    VOLUME = 	"35",
    PAGES = 	"335-356"}

@Article{casda1991,
    AUTHOR = 	"Casdagli, M.",
    TITLE = 	"Nonlinear prediction of chaotic time series",
    YEAR = 	"1991",
    JOURNAL = 	"Physica D",
    VOLUME = 	"20",
    PAGES = 	"335-356"}

@article{chich2009,
  title = {Reliable detection of directional couplings using rank statistics},
  author = {Chicharro, Daniel and Andrzejak, Ralph G.},
  journal = {Phys. Rev. E},
  volume = {80},
  issue = {2},
  pages = {026217},
  numpages = {5},
  year = {2009},
  month = {Aug},
  doi = {10.1103/PhysRevE.80.026217},
  url = {http://link.aps.org/doi/10.1103/PhysRevE.80.026217},
  publisher = {American Physical Society}
}

@Article{cirel1999,
  AUTHOR = 	"Cirelli, Ch. and others",
  TITLE = 	"No evidence of brain cell degeneration after long - term sleep deprivation in rats",
  YEAR = 	"1999",
  JOURNAL = 	"Brain Research	",
  VOLUME = 	"840",
  PAGES = 	"184-193"}

@Article{corsi1996,
  AUTHOR = 	"Corsi-Cabrera, M. and Arce, C. and Ramos, J. and Lorenzo, I. and Guevara, M. A.",
  TITLE = 	"Time course of reaction time and {EEG} while performing a vigilance task during total sleep deprivation",
  YEAR = 	"1996",
  JOURNAL = 	"Sleep",
  VOLUME = 	"19",
  NUMBER = "7",
  PAGES = 	"563-569"}
    

@Article{corsi2006,
  AUTHOR = 	"Corsi-Cabrera, M. and Mu{\~n}oz-Torres, Z. and del R?o-Portilla, Y. and Guevara, M. A.",
  TITLE = 	"Power and coherent oscillations distinguish {REM} sleep, stage 1 and wakefulness",
  YEAR = 	"2006",
  JOURNAL = 	"International Journal of Psychophysiology",
  VOLUME = 	"60",
  NUMBER = "1",
  PAGES = 	"59-66"}
  
@book{cover2012,
  title={Elements of information theory},
  author={Cover, Thomas M and Thomas, Joy A},
  year={2012},
  publisher={John Wiley \& Sons}
}

@article{cummi2015,
  title = "On the Efficacy of State Space Reconstruction Methods in Determining Causality",
  author = "Cummins, Bree and Gedeon, Tom\'{a}\v{s} and Spendlove, Kelly",
  journal = "SIAM Journal on Applied Dynamical Systems",
  volume = "14",
  number = "1",
  pages = "335-381",
  year = "2015",
  publisher = "SIAM"}

@Article{daan1984,
  AUTHOR = 	"Daan, S. and Beersma, D. G. M. and Borb\'{e}ly, A. A.",
  TITLE = 	"Timing of human sleep: recovery process gated by a circadian pacemaker",
  YEAR = 	"1984",
  JOURNAL = 	"American Journal of Physiology -- Regulatory, Integrative and Comparative Physiology",
  VOLUME = 	"246",
  PAGES = 	"161-178"}  

@Article{danke2004,
  AUTHOR = "Danker-Hopfe, H. and Kunz, D. and Gruber, G. and Kl{\"o}sch, G. and Lorenzo, J. L. and Himanen, S. L. and Kemp, B. and Penzel, T. and R{\"o}schke, J. and Dorn, H. and Schl{\"o}gl, A. and  Trenker, E. and Dorffner, G.",
  TITLE = "Interrater reliability between scorers from eight {E}uropean sleep laboratories in subjects with different sleep disorders",
  YEAR = "2004",
  JOURNAL = "Journal of Sleep Research",
  VOLUME = "13",
  NUMBER = "1",
  PAGES = "63-69"}


@Article{degen2004,
  AUTHOR = 	"De Gennaro, L. and Vecchio, F. and Ferrara, M. and Curcio, G. and Rossini, P. M. and Babiloni, C.",
  TITLE = 	"Changes in fronto-posterior functional coupling at sleep onset in humans",
  YEAR = 	"2004",
  JOURNAL = 	"Journal of Sleep Research",
  VOLUME = 	"13",
  NUMBER = 	"3",
  PAGES = 	"209-217"}  

@Article{demen1957,
  AUTHOR = 	"Dement, W. C. and Kleitman, N.",
  TITLE = 	"Cyclic variations in {EEG} during sleep and their relation to eye movements, body motility, and dreaming",
  YEAR = 	"1957",
  JOURNAL = 	"Electroencephalogr Clin Neurophysiol   ",
  VOLUME = 	"9",
  NUMBER = "4",
  PAGES = 	"673-690"}

@Article{dijk1989,
  AUTHOR = 	"Dijk, D. J. and Beersma, D. G. and van den Hoofdakker, R. H.",
  TITLE = 	"All night spectral analysis of {EEG} sleep in young adult and middle-aged male subjects",
  YEAR = 	"1989",
  JOURNAL = 	"Neurobiol Aging",
  VOLUME = 	"10(6)",
  PAGES = 	"677-682"}

@article{dimat2003,
  title={Scaling behaviors in differently developed markets},
  author={Di Matteo, Tiziana and Aste, Tomaso and Dacorogna, MM},
  journal={Physica A: Statistical Mechanics and its Applications},
  volume={324},
  number={1},
  pages={183--188},
  year={2003},
  publisher={Elsevier}
}

@Article{doghr1997,
  AUTHOR = 	"Doghramnji, K. and others",
  TITLE = 	"A Normative Study of the Maintenance of Wakefulness Test (MWT)",
  YEAR = 	"1997",
  JOURNAL = 	"Electroncephalogr. Clin. Neurophysiol.	",
  VOLUME = 	"103",
  PAGES = 	"554-562"}

@Article{domin2007,
	AUTHOR = "Dom\'{i}nguez, L. G. and Wennberg, R. and Vel\'{a}zquez, J. L. P. and   Guevara, R.",
	TITLE = "Enhanced measured synchronization of unsynchronized sources: inspecting the physiological significance of synchronization analysis of whole brain electrophysiological recordings",	
	JOURNAL = "International Journal of Physical Sciences",
	VOLUME = "2",
	NUMBER = "11",
	YEAR = "2007",
	PAGES = "305-317"
}

@Article{duckr2005,
  AUTHOR = 	"Duckrow, R. B. and Zaveri, H. P.",
  TITLE = 	"Coherence of the electroencephalogram during the first sleep cycle",
  YEAR = 	"2005",
  JOURNAL = 	"Clin Neurophysiol",
  VOLUME = 	"116",
  NUMBER = "5",
  PAGES = 	"1088-1095"}

@Article{dumer1981,
	AUTHOR = "Dumermuth, G. and Lehmann, D.",
	TITLE = "{EEG} {P}ower and {C}oherence during {N}on-{REM} and {REM} {P}hases in {H}umans in {A}ll-{N}ight {S}leep {A}nalyses",
	YEAR = "1981",
	JOURNAL = "Eur Neurol ",
	VOLUME = "20",
	NUMBER = "6",
	PAGES = "429-434"
}
    
@Article{dumer1983,
	AUTHOR = "Dumermuth, G. and Lange, B and Lehmann, D. and Meier, C. A. and Dinkelmann, R. and Molinari, L.",
	TITLE = "{S}pectral {A}nalysis of {A}ll-{N}igth {S}leep {EEG} in {H}ealthy {A}dults",
	YEAR = "1983",
	JOURNAL = "Eur Neurol ",
	VOLUME = "22",
	NUMBER = "5",
	PAGES = "322-339"
}

@Article{durka1999,
   AUTHOR = 	"Durka, P.J. and Ksi??yk, R. and Blinowska, K.J.",
   TITLE = 	"Neural networks and wavelet analysis in {EEG} artefact recognition",
   YEAR = 	"1999",
   JOURNAL = 	"II Konferencja Sieci Neuronowe i Ich Zastosowania, Szczyrk",
   VOLUME = 	"",
   PAGES = 	"1996"}
   
@Article{ehler1998,
   AUTHOR = 	"Ehlers, C. L. and Kupfer, D. J. and Buysse, D. J. and Cluss, P. A. and Miewald, J. M. and Bisson, E. F. and Grochocinski, V. J.",
   TITLE = 	"The {P}ittsburgh study of normal sleep in young adults: focus on the relationship between waking and sleeping {EEG} spectral patterns",
   YEAR = 	"1998",
   JOURNAL = 	"Electroencephalogr Clin Neurophysiol ",
   VOLUME = 	"106(3)",
   PAGES = 	"199-205"}

@article{eke2002,
  title={Fractal characterization of complexity in temporal physiological signals},
  author={Eke, Andras and Herman, Peter and Kocsis, L and Kozak, LR},
  journal={Physiological measurement},
  volume={23},
  number={1},
  pages={R1},
  year={2002},
  publisher={IOP Publishing}
}

@Article{elul1969,
  AUTHOR = 	"Elul, R.",
  TITLE =	"Gaussian behavior of the electroencephalogram: {C}hanges during performance of mental task",
  JOURNAL =	"Science",
  VOLUME =	"164",
  NUMBER = "3877",
  YEAR =	"1969",
  PAGES =	"328-331"}
  
@Article{elul1975,
  AUTHOR = 	"Elul, R. and Hanley, J. and Simmons, J., Q.",
  TITLE =	"Non-{G}aussian behavior of the {EEG} in {D}own's syndrome suggests decreased neuronal connections",
  JOURNAL =	"Acta Neurologica Scandinavica",
  VOLUME =	"51",
  NUMBER = "1",
  YEAR =	"1975",
  PAGES =	"21-28"}

@Article{ernst2004,
	AUTHOR = "Ernst, M. D.",
	TITLE = "Permutation Methods: A Basis for Exact Inference",	
	JOURNAL = "Statistical Science",
	VOLUME = "19",
	NUMBER = "4",
	YEAR = "2004",
	PAGES = "676-685"
}

@article{estel2001,
  title={A comparison of waveform fractal dimension algorithms},
  author={Esteller, Rosana and Vachtsevanos, George and Echauz, Javier and Litt, Brian},
  journal={Circuits and Systems I: Fundamental Theory and Applications, IEEE Transactions on},
  volume={48},
  number={2},
  pages={177--183},
  year={2001},
  publisher={IEEE}
}  

@Article{estev2000,
   AUTHOR = 	"Est\'{e}vez, P. A. and Fern{\'a}ndez, M. and Held, C. and Holzmann, C. and P{\'e}rez, C. and P{\'e}rez, J.P.",
   TITLE = 	"Classification of {S}leep-{W}aking {S}tates using {M}odular {N}eural {N}etworks",
   Journal = 	"2000 IEEE International Conference on Systems, Man, and Cybernetics",
   VOLUME = "4",
   YEAR = 	"2000",
   PAGES = 	"2580-2585"}
   
  
@Article{estev2002,
   AUTHOR = 	"Est\'{e}vez, P. A. and Held, C. and Holzmann, C. and P{\'e}rez, C. and P{\'e}rez, J.P. and Heiss, J. and Garrido, M. and Peirano, P.",
   TITLE = 	"Polysomnographic pattern recognition for automated classification of sleep-waking states in infants",
   YEAR = 	"2002",
   JOURNAL = 	"	Medical and Biological Engineering and Computing",
   VOLUME = 	"40",
   NUMBER = "1",
   PAGES = 	"105-113"}

@Article{evans1992,
   AUTHOR = 	"Evans B. M.",
   TITLE = 	"Periodic activity in cerebral arousal mechanisms--the relationship to sleep and brain damage",
   YEAR = 	"1992",
   JOURNAL = 	"Electroencephalogr Clin Neurophysiol   ",
   VOLUME = 	"83(2)",
   PAGES = 	"130-137"}
   
@Article{evans1993,
   AUTHOR = 	"Evans B. M.",
   TITLE = 	"Cyclical activity in non-rapid eye movement sleep: a proposed arousal inhibitory mechanism",
   YEAR = 	"1993",
   JOURNAL = 	"Electroencephalogr Clin Neurophysiol   ",
   VOLUME = 	"86(2)",
   PAGES = 	"123-131"}
   
@Article{farme1987,
    AUTHOR = 	"Farmer, J. D. and Sidorowich, J.J.",
    TITLE = 	"Predicting Chaotic Time Series	",
    YEAR = 	"1987",
    JOURNAL = 	"Phys Rev Lett",
    VOLUME = 	"59",
    PAGES = 	"845-848"}

@Article{fein1988,
	AUTHOR = "Fein, G. and  Raz, J. and Brown, F. F. and Merrin, E. L.",
	TITLE = "Common reference coherence data are confounded by power and phase effects",	
	JOURNAL = "Electroencephalogr Clin Neurophysiol ",
	VOLUME = "69",
	NUMBER = "6",
	YEAR = "1988",
	PAGES = "581-584"
}

@Article{fell1996,
  AUTHOR = 	"Fell, J. and R{\"o}schke, J. and Mann, K. and Sch{\"a}ffner, C.",
  TITLE = 	"Discrimination of sleep stages: a comparison between spectral and nonlinear {EEG}              measures",
  YEAR = 	"1996",
  JOURNAL = 	"Electroencephalogr Clin Neurophysiol   ",
  VOLUME = 	"98",
  NUMBER = "5",
  PAGES = 	"401-410"}

@Article{fell2000,
  AUTHOR = 	"Fell, J. and Mann, K. and R{\"o}schke, J. and Gopinathan, M. S.",
  TITLE = 	"Nonlinear analysis of continuous {ECG} during sleep {II}. {D}ynamical measures",
  YEAR = 	"2000",
  JOURNAL = 	"Biological Cybernetics",
  VOLUME = 	"82",
  NUMBER = "6",
  PAGES = 	"485-491"}

@Article{ferri2000,
    AUTHOR = 	"Ferri, R. and Elia, M. and Musumeci, S.A. and Pettinato S.",
    TITLE = 	"The time course of frequency bands (15-45 Hz) in all-night spectral analysis of sleep {EEG}",
    YEAR = 	"2000",
    JOURNAL = 	"Clin Neurophysiol",
    VOLUME = 	"111",
    PAGES = 	"1258-1265"}

@Article{flexe2005,
    AUTHOR = 	"Flexer, A. and Gruber, G. and Dorffner, G.",
    TITLE = 	"A reliable probabilistic sleep stager based on a single {EEG} signal",
    YEAR = 	"2005",
    JOURNAL =  "Artificial Intelligence in Medicine",
    VOLUME = 	"33",
    NUMBER = "3",
    PAGES = 	"199-207"}

@Article{gabor1946,
	AUTHOR = "Gabor, D.",
	TITLE = "Theory of communication",	
	JOURNAL = "J. IEE",
	VOLUME = "93",
	NUMBER = "",
	YEAR = "1946",
	PAGES = "429-457"
}
  
@Article{gaill1973,
    AUTHOR = 	"Gaillard, J. M. and Tissot, R.",
    TITLE = 	"Principles of automatic analysis of sleep records with a hybrid system",
    YEAR = 	"1973",
    JOURNAL = 	"Computers and Biomedical Research",
    VOLUME = 	"6",
    NUMBER = "1",
    PAGES = 	"1-13"}

@Article{galbr1993,
    AUTHOR = 	"Galbraith, G. C. and Wong, E.",
    TITLE = 	"Moment Analysis of {EEG} Amplitude Histograms and Spectral Analysis: Relative Classification of 	    Several Behavioral Tasks",
    YEAR = 	"1993",
    JOURNAL = 	"Perceptual and Motor Skills",
    VOLUME = 	"76",
    PAGES = 	"859-866"}
    
@Book{galka2000,
  AUTHOR = 	"Galka, A.",
  TITLE = 	"Topics in Nonlinear Time Series Analysis",
  YEAR = 	"2000",
  PUBLISHER = 	"World Scientific"}

@Inproceedings{gevin1987,
    EDITOR = "Gevins, A. S. and R\'{e}mond, A.",
    AUTHOR =	"Dumermuth, G. and Molinari, L.",
    BOOKTITLE = "Handbook of Electroencephalography and clinical Neurophysiology. Methods of Analysis of Brain Electrical and Magnetic Signals",
    TITLE =	"Spectral {A}nalysis of {EEG} {B}ackground {A}ctivity",
    YEAR = 	"1987",
    PUBLISHER =	"Elsevier, Amsterdam",
    PAGES = 	"85-130"}

@Article{giona1991,
    AUTHOR = 	"Giona,M. and Lentini,F. and Cimagalli, V.",
    TITLE = 	"Functional reconstruction and local prediction of chaotic time series	",
    YEAR = 	"1991",
    JOURNAL = 	"Phys. Review A	",
    VOLUME = 	"44",
    NUMBER = "6",
    PAGES = 	"3496-3502"}

@Article{glass1983,
    AUTHOR = 	"Glass, L. and Guevara, M.R. and Shrier, A.",
    TITLE = 	"Bifurcation and chaos in a periodically stimulated cardiac oscillator",
    YEAR = 	"1983",
    JOURNAL = 	"Physica D",
    VOLUME = 	"7",
    PAGES = 	"89-101"}

@Article{goldb2002,
AUTHOR = "Goldberger, A. L. and Amaral, L. A. N. and Hausdorff, J. M. and  Ivanov, P. Ch. and Peng, C.-K. and Stanley, H. E.",
TITLE = "Fractal dynamics in physiology: Alterations with disease and aging",
JOURNAL = "Proceedings of the National Academy of Sciences of the United States of America ",
VOLUME = "99", 
NUMBER = "1", 
YEAR = "2002",
PAGES = "2466-2472"
}

@article{grang1969,
  title={Investigating causal relations by econometric models and cross-spectral methods},
  author={Granger, Clive WJ},
  journal={Econometrica: Journal of the Econometric Society},
  pages={424--438},
  year={1969},
  publisher={JSTOR}
}
    
@Article{grass1983,
    AUTHOR = 	"Grassberger, P. and Procaccia, I.",
    TITLE = 	"Measuring the strangeness of strange attractors",
    YEAR = 	"1983",
    JOURNAL = 	"Physica D",
    VOLUME = 	"9",
    NUMBER = "1-2",
    PAGES = 	"189-208"}
  
@Article{grass1993,
    AUTHOR = 	"Grassberger, P. and others",
    TITLE = 	"On noise reduction methods for chaotic data",
    YEAR = 	"1993",
    JOURNAL = 	"Chaos",
    VOLUME = 	"3",
    PAGES = 	"127-141"}

@Article{gray1989,
	AUTHOR = "Gray, Ch. M. and K{\"o}nig, P. and Engel, A. K. and Singer, W.",
	TITLE = "Oscillatory responses in cat visual cortex exhibit inter-columnar synchronization which reflects global stimulus properties",	
	JOURNAL = "Nature",
	VOLUME = "338",
	NUMBER = "",
	YEAR = "1989",
	PAGES = "334-337"
}

@Article{gueva2005,
	AUTHOR = "Guevara, R. and Velazquez, J. L. P. and Nenadovic, V. and Wennberg, R. and Senjanovi\'{c}, G. and Dominguez, L. G.",
	TITLE = "Phase Synchronization Measurements Using Electroencephalographic Recordings What Can We Really Say About Neuronal Synchrony?",	
	JOURNAL = "Neuroinformatics",
	VOLUME = "3",
	NUMBER = "4",
	YEAR = "2005",
	PAGES = "301-314"
}

@Article{hakki1993,
  AUTHOR = 	"H{\"a}kkinen, V. and Hirvonen, K. and Hasan, J. and Kataja, M. and V{\"a}rri, A. and Loula, P. and Eskola, H.",
  TITLE =	"The effect of small differences in electrode position on {{EOG}} signals: application to vigilance studies ",
  JOURNAL =	"Electroencephalogr Clin Neurophysiol ",
  VOLUME =	"86",
  NUMBER  = "4",
  YEAR =	"1993",
  PAGES =	"294-300"}
    
@Article{halas2004,
  AUTHOR = 	"Hal\'{a}sz, P. and others",
  TITLE = 	"The nature of arousal in sleep",
  YEAR = 	"2004",
  JOURNAL = 	"J. Sleep Res.",
  VOLUME = 	"13",
  PAGES = 	"1-23"}

@Article{hasan1996,
  AUTHOR = 	"Hasan, J.",
  TITLE = 	"Past and {F}uture of {C}omputer-{A}ssisted {S}leep {A}nalysis and {D}rowsiness {A}ssessment",
  YEAR = 	"1996",
  JOURNAL = 	"Journal of Clinical Neurophysiology.",
  VOLUME = 	"13",
  NUMBER = "4",
  PAGES = 	"295-313"}
 
@Article{harpe1987,
  AUTHOR = 	"Harper, R. M. and Schechtman, V. L. and Kluge, K. A.",
  TITLE = 	"Machine classification of infant sleep state using cardiorespiratory measures",
  YEAR = 	"1987",
  JOURNAL = 	"Electroencephalogr Clin Neurophysiol   ",
  VOLUME = 	"67",
  NUMBER = "4",	
  PAGES = 	"379-387"}

@Article{hegge1999,
	AUTHOR = "Hegger, R. and Kantz, H.",
	TITLE = "Improved false nearest neighbor method to detect determinism in time series data",	
	JOURNAL = "Phys Rev E",
	VOLUME = "60",
	NUMBER = "4",
	YEAR = "1999",
	PAGES = "4970-4973"
}

@Article{hegge1999b,
	AUTHOR = "Hegger, R. and Kantz, H. and Schreiber, T,",
	TITLE = "Practical implementation of nonlinear time series methods: The TISEAN package",	
	JOURNAL = "	Chaos: An Interdisciplinary Journal of Nonlinear Science",
	VOLUME = "9",
	NUMBER = "2",
	YEAR = "1999",
	PAGES = "413-435"
}

@Article{herna1995,
    AUTHOR = 	"Hern\'{a}ndez, J. L. and others",
    TITLE = 	"{EEG} predictability: adequacy of non-linear forecasting methods",
    YEAR = 	"1995",
    JOURNAL = 	"Int. J. of Bio-Medical Computing",
    VOLUME = 	"38",
    PAGES = 	"197-206"}

@Article{higuc1988,
  AUTHOR = 	"Higuchi, T.",
  TITLE =	"Approach to an {I}rregular {T}ime {S}eries on the {B}asis of the {F}ractal {T}heory",
  JOURNAL =	"Physica D",
  VOLUME =	"31",
  NUMBER = "2",
  YEAR =	"1988",
  PAGES =	"277-283"}

@Article{higuc1990,
  AUTHOR = 	"Higuchi, T.",
  TITLE =	"Relationship between the fractal dimension and the power law index for a time series: a numerical investigation",
  JOURNAL =	"Physica D",
  VOLUME =	"46",
  YEAR =	"1990",
  NUMBER = "2",
  PAGES =	"254-264"}

@PHDTHESIS{himan2000,
  AUTHOR = 	"Himanen, S.-L."	,
  TITLE = 	"A {N}ew {V}isual {A}daptive {S}coring {S}ystem for {S}leep {R}ecordings",
  SCHOOL = 	"Universitatis Tamperensis",
  YEAR = 	"2000"}

 
@Article{hori1985,
    AUTHOR = 	"Hori, T.",
    TITLE = 	"Spatiotemporal changes of {EEG} activity during waking-sleeping transition period",
    YEAR = 	"1985",
    JOURNAL = 	"International Journal of Neuroscience",
    VOLUME = 	"27",
    NUMBER = "1",
    PAGES = 	"101-114"}

@Article{horne1997,
    AUTHOR = 	"Horne, J.",
    TITLE = 	"The Phenomena of Human Sleep",
    YEAR = 	"1997",
    JOURNAL = 	"Karger Gazette	",
    VOLUME = 	"61",
    PAGES = 	""}

@Article{huber2004,
    AUTHOR = 	"Huber, R. and Ghilardi, M. F. and Massimini, M. and Tononi, G.",
    TITLE = 	"Local sleep and learning",
    YEAR = 	"2004",
    JOURNAL = 	"Nature",
    VOLUME = 	"430",
    PAGES = 	"78-81"}

@article{hurst1951,
  title={$\{$Long-term storage capacity of reservoirs$\}$},
  author={Hurst, Harold Edwin},
  journal={Trans. Amer. Soc. Civil Eng.},
  volume={116},
  pages={770--808},
  year={1951}
}

@Book{iber2007,
  AUTHOR = 	"Iber, C. and Ancoli-Israel, S. and Chesson, A. and Quan, S.",
  TITLE = 	"The AASM Manual for the Scoring of Sleep and Associated Events: Rules,
Terminology, and Technical Specifications",
  YEAR = 	"2007",
  PUBLISHER = 	"Westchester, Illinois: American Academy of Sleep Medicine"}
  
@Article{inouy1991,
	AUTHOR = "Inouye, T.  and Shinosaki, K.  and Sakamoto, H.  and Toi, S.  and Ukai, S.  and Iyama, A.  and Katsuda Y.  and Hirano, M. ",
	TITLE = "Quantification of {EEG} irregularity by use of the entropy of the power spectrum",	
	JOURNAL = "Electroencephalogr Clin Neurophysiol ",
	VOLUME = "79",
	NUMBER = "3",
	YEAR = "1991",
	PAGES = "204-210"
}

@article{janja2008,
  title={An approach for characterizing coupling in dynamical systems},
  author={Janjarasjitt, S and Loparo, KA},
  journal={Physica D: Nonlinear Phenomena},
  volume={237},
  number={19},
  pages={2482--2486},
  year={2008},
  publisher={Elsevier}
}

@Article{janse1989,
    AUTHOR = 	"Jansen, B. H. and  Dawant, B. M.",
    TITLE = 	"Knowledge-based approach to sleep {EEG} analysis-a feasibility study",
    YEAR = 	"1989",
    JOURNAL = "IEEE Transactions on Biomedical Engineering",
    VOLUME = 	"36",
    NUMBER = "5",
    PAGES = 	"510-518"}

@Article{jober1992,
    AUTHOR = 	"Jobert, M. and Poiseau, E. and J{\"a}hnig, P. and Schulz, H. and Kubicki, S.",
    TITLE = 	"Topographical analysis of sleep spindle activity",
    YEAR = 	"1992",
    JOURNAL = 	"Neuropsychobiology",
    VOLUME = 	"26",
    NUMBER = "4",
    PAGES = 	"210-217"}
 
@Article{johns1969,
    AUTHOR = 	"Johnson, L. and Lubin, A. and Naitoh, P. and Nute, C. and Austin, M.",
    TITLE = 	"Spectral analysis of the {EEG} of dominant and non-dominant alpha subjects during waking and sleeping",
    YEAR = 	"1969",
    JOURNAL = 	"Electroencephalogr Clin Neurophysiol   ",
    VOLUME = 	"26",
    NUMBER = "4",
    PAGES = 	"361-370"}   

@Article{kamin1997,
	AUTHOR = "Kami{\"n}ski, M. and Blinowska, K. and Szelenberger, W.",
	TITLE = "Topographic analysis of coherence and propagation of {EEG} activity during sleep and wakefulness",	
	JOURNAL = "Electroencephalography and clinical physiology",
	VOLUME = "102",
	NUMBER = "3",
	YEAR = "1997",
	PAGES = "216-227"
}

@Book{kantz1997,
  AUTHOR = 	"Kantz, H. and Schreiber T.",
  TITLE = 	"Nonlinear Time Series Analyses",
  YEAR = 	"1997",
  PUBLISHER = 	"Cambridge University Press"}
  
@Article{kelle1985,
  AUTHOR = "Kelley, J. T. and Reilly, E. L. and Overall, J. E. and Reed, K.",
  TITLE = "Reliability of rapid clinical staging of all night sleep {EEG}",
  YEAR = "1985",
  JOURNAL = "Clinical Electroencephalography",
  VOLUME = "16",
  NUMBER = "1",
  PAGES = "16-20"}

@Article{kenne1992,
	AUTHOR = "Kennel, M. B. and Brown, R. and Abarbanel, H. D. I.",
	TITLE = "Determining embedding dimension for phase-space reconstruction using a geometricial construction",	
	JOURNAL = "Phys Rev A",
	VOLUME = "45",
	NUMBER = "69",
	YEAR = "1992",
	PAGES = "3403-3411"
}
    
@Article{klosc2001,
  AUTHOR = 	"Kl{\"o}sch, G and Kemp, B. and Penzel, T. and Schl{\"o}gl, A. and Rappelsberger, P. and Trenker, E. and Gruber, G. and Zeitlhofer, J. and Saletu, B. and Herrmann, W.M. and Himanen, S.L. and Kunz, D. and Barbanoj, M.J. and R{\"o}schke, J. and V{\"a}rri, A. and Dorffner, G.",
  TITLE = 	"The {SIESTA} project polygraphic and clinical database",
  YEAR = 	"2001",
  JOURNAL = 	"IEEE Engineering in Medicine and Biology Magazine",
  VOLUME = 	"20",
  NUMBER = "3",
  PAGES = 	"51-57"}
        
@Article{kobay1999,
  AUTHOR = 	"Kobayashi, T. and others",
  TITLE = 	"Non-linear analysis of the sleep {EEG}",
  YEAR = 	"1999",
  JOURNAL = 	"Psychiatry and Clinical Neurosciences",
  VOLUME = 	"53",
  NUMBER = "2",
  PAGES = 	"159-162"}
   
@Article{kobay2002,
    AUTHOR = 	"Kobayashi, T. and Madokoro, S. and Misaki, K. and Murayama, J. and Nakagawa, H. and Wada, Y.",
    TITLE = 	"Human Sleep Physiology. {I}nterhemispheric differences of the correlation dimension in a human sleep electroencephalogram",
    YEAR = 	"2002",
    JOURNAL = 	"Psychiatry and Clinical Neurosciences",
    VOLUME = 	"56",
    PAGES = 	"265-266"}

@Article{koste1993,
  AUTHOR = 	"Kostelich, E. J. and Schreiber, T.",
  TITLE = 	"Noise reduction in chaotic time-series data: A survey of common methods",
  YEAR = 	"1993",
  JOURNAL = 	"Phys Rev E",
  VOLUME = 	"48",
  NUMBER = 	"3",
  PAGES = 	"1752-1763"}

@Article{kojim1981,
    AUTHOR = 	"Kojima, T. and others",
    TITLE = 	"Eye movement as an indicator of brain function",
    YEAR = 	"1981",
    JOURNAL = 	"Folia Psychiatr Neurol Jpn.",
    VOLUME = 	"35(4)",
    PAGES = 	"425-435"}  
    
@Article{krako1995,
    AUTHOR = "Krakovsk\'{a}, A.",
    TITLE = "Spectral decay vs. correlation dimension of {EEG}",
    YEAR = "1995",
    JOURNAL = "Acta physica slovaca",
    VOLUME = "45",
    NUMBER = "5",
    PAGES = "567-574"}
 
@Article{krako2008,
    AUTHOR = 	"Krakovsk\'{a}, A. and \v{S}tolc, S.",
    TITLE =  "Spectral decay vs. correlation dimension of {EEG}",
    JOURNAL = "Neurocomputing",
    YEAR = "2008",
    VOLUME = "71",
    NUMBER = "13--17",
    PAGES = "2978--2985"
}

@inproceedings{krako2013,
  title={Interdependence Measure Based on Correlation Dimension},
  author={Krakovsk{\'a}, Anna and Bud{\'a}{\v{c}}ov{\'a}, Hana},
  booktitle={Proceedings of the 9th International Conference on Measurement},
  pages={31--34},
  year={2013},
  organization={ISBN 978-80-969-672-5-4}
}

@article{krako2015,
  title={Use of False Nearest Neighbours for Selecting Variables and Embedding Parameters for State Space Reconstruction. Article ID 932750},
  author={Krakovsk{\'a}, Anna and Mezeiov{\'a}, Krist{\'\i}na and Bud{\'a}{\v{c}}ov{\'a}, Hana},
  journal={Journal of Complex Systems},
  volume={2015},
  year={2015},
  publisher={Hindawi Publishing Corporation}
} 

@misc{1511.00505,
  author = {Anna Krakovsk� and Jozef Jakub�k and Hana Bud��ov� and M�ria Holecyov�},
  title = {{C}ausality studied in reconstructed state space. {E}xamples of uni-directionally connected chaotic systems},
  year = {2015},
  eprint = {1511.00505},
  note = {arXiv:1511.00505v1}
}

@article{kreuz2007,
  title={Measuring synchronization in coupled model systems: A comparison of different approaches},
  author={Kreuz, Thomas and Mormann, Florian and Andrzejak, Ralph G and Kraskov, Alexander and Lehnertz, Klaus and Grassberger, Peter},
  journal={Physica D: Nonlinear Phenomena},
  volume={225},
  number={1},
  pages={29--42},
  year={2007},
  publisher={Elsevier}
}

@Article{krzan1977,
  AUTHOR = 	"Krzanowski, W. J.",
  TITLE =	"The {P}erformance of {F}isher's {L}inear {D}iscriminant {F}unction under {N}on-{O}ptimal {C}onditions",
  JOURNAL =	"Technometrics",
  VOLUME =	"19",
  NUMBER = "2",
  YEAR =	"1977",
  PAGES =	"191-200"}
  
@INCOLLECTION{kubic1985,
    AUTHOR =	"Kubicki, S. and Herrmann, W. M. and H{\"o}ller, L.",
    TITLE =	"Critical comments on the rules by {R}echtschaffen and {K}ales concerning the visual evaluation of {EEG} sleep records",
    BOOKTITLE = "Methods of Sleep Research",
    EDITOR = "Kubicki, S. and Herrmann, W. M.",
    YEAR = 	"1985",
    PUBLISHER =	"Gustav Fischer Verlag, Stuttgart, New York",
    PAGES = "19-35"}

@Article{kubic1989,
    AUTHOR = 	"Kubicki, S. and  H{\"o}ller, L. and Berg, I. and Pastelak-Price, C. and Dorow, R.",
    TITLE = 	"Sleep {EEG} evaluation: a comparison of results obtained by visual scoring and automatic analysis with the {O}xford sleep stager",
    YEAR = 	"1989",
    JOURNAL = 	"Sleep",
    VOLUME = 	"12",
    NUMBER ="2",
    PAGES = 	"140-149"}

@Article{lacha1999,
	AUTHOR = "Lachaux, J.-P. and Rodriguez, E. and Martinerie, J. and Varela, F. J. ",
	TITLE = "Measuring Phase Synchrony in Brain Signals",	
	JOURNAL = "Hum Brain Mapp",
	VOLUME = "8",
	NUMBER = "4",
	YEAR = "1999",
	PAGES = "194-208"
}

@Book{laros2006,
  AUTHOR = 	"Larose, D.",
  TITLE = 	"Data Mining Methods and Models",
  YEAR = 	"2006",
  PUBLISHER = 	"Wiley InterScience"
}

@article{lee2012,
  title={Transfer entropy estimation and directional coupling change detection in biomedical time series},
  author={Lee, Joon and Nemati, Shamim and Silva, Ikaro and Edwards, Bradley A and Butler, James P and Malhotra, Atul and others},
  journal={Biomed. Eng},
  year={2012}
}

@article{levan1999,
  title={Nonlinear analyses of interictal EEG map the brain interdependences in human focal epilepsy},
  author={Le Van Quyen, Michel and Martinerie, Jacques and Adam, Claude and Varela, Francisco J},
  journal={Physica D: Nonlinear Phenomena},
  volume={127},
  number={3},
  pages={250--266},
  year={1999},
  publisher={Elsevier}
}

@Article{levan2001,
	AUTHOR = "Le Van Quyen, M. and Foucher, J. and Lachaux J.-P. and Rodriguez, E. and Lutz, A. and Martinerie, J. and Varela, F. J. ",
	TITLE = "Comparison of {H}ilbert transform and wavelet methods for the analysis of neuronal synchrony",	
	JOURNAL = "J Neurosci Methods",
	VOLUME = "111",
	NUMBER = "2",
	YEAR = "2001",
	PAGES = "83-98"
}

@Article{levan2003,
    AUTHOR = 	"Le Van Quyen, M. and Chavez, M. and Rudrauf, D. and Martinerie, J.",
    TITLE = 	"Exploring the nonlinear dynamics of the brain",
    YEAR = 	"2003",
    JOURNAL = 	"Journal of Physiology-Paris",
    VOLUME = 	"97",
    NUMBER = "4-6",
    PAGES = 	"629-639"}

@Article{letel1998,
    AUTHOR = 	"Letellier, C. and Maquet, J. and Le Sceller, L. and Gouesbet, G. and Aguirre, L.A.",
    TITLE = 	"On the non-equivalence of observables in phase-space reconstructions from recorded time series",
    YEAR = 	"1998",
    JOURNAL = 	"J. Phys. A: Math. Gen.",
    VOLUME = 	"31",
     PAGES = 	"7913-7927"}

@Article{letel2002,
    AUTHOR = 	"Letellier, C. and Aguirre, L.A.",
    TITLE = 	"Investigating nonlinear dynamics from time series: The influence of symmetries and the choice of observables",
    YEAR = 	"2002",
    JOURNAL = 	"Chaos",
    VOLUME = 	"12",
    NUMBER = "3",
    PAGES = 	"549-558"}

@Article{letel2005,
    AUTHOR = 	"Letellier, C. and Aguirre, L.A. and Maquet, J.",
    TITLE = 	"Relation between observability and differential embeddings for nonlinear dynamics",
    YEAR = 	"2005",
    JOURNAL = 	"Physical Review E",
    VOLUME = 	"71",
     PAGES = 	"066213"}

@Article{letel2009,
    AUTHOR = 	"Letellier, C. and Aguirre, L.A.",
    TITLE = 	"Symbolic observability coefficients for univariate and multivariate analysis",
    YEAR = 	"2009",
    JOURNAL = 	"Physical Review E",
    VOLUME = 	"79",
     PAGES = 	"066210"}

@Article{linke2001,
    AUTHOR = 	"Linkenkaer-Hansen, K. and Nikouline, V. V. and Palva, M. J. and Ilmoniemi, R. J.",
    TITLE = 	"Long-Range Temporal Correlations and Scaling Behavior in Human Brain Oscillations",
    YEAR = 	"2001",
    JOURNAL = 	"J Neurosci",
    VOLUME = 	"21",
    NUMBER  = "4",
    PAGES = 	"1370-1377"}

@incollection{littl2006,
   Author = {Little, M. and McSharry, P. and Moroz, I. and Roberts, S.},
   Title = {Nonlinear, Biophysically-Informed Speech Pathology Detection},
   BookTitle = {2006 IEEE International Conference on Acoustics, Speech and Signal Processing},
   Volume = {2},
   Year = {2006} }

@Article{loomi1937,
  AUTHOR = 	"Loomis, A.L. and Harvey, E.N. and Hobart, G.A"	,
  TITLE = 	"Cerebral States During Sleep, as Studied by Human Brain Potentials",
  YEAR = 	"1937",
  JOURNAL = 	"Journal of Experimental Psychology",
  VOLUME = 	"21",
  PAGES = 	"127-144"}

@Article{loren1991,
  AUTHOR = 	"Lorenz E. N."	,
  TITLE = 	"Dimension of weather and climate attractors",
  YEAR = 	"1991",
  JOURNAL = 	"Nature",
  VOLUME = 	"353",
  PAGES = 	"241-244",}
%
%@article{lutz2009,
%  title = {Granger Causality Test - Matlab Function},
%  author = {Lutz, C.},
%  journal = {},
%  volume = {},
%  issue = {},
%  pages = {},
%  year = {2009},
%  url = ''http://www.mathworks.com/matlabcentral/fileexchange/25467-granger-causality-test/content/granger_cause.m'',
%}

@Book{mande1977,
  AUTHOR = 	"Mandelbrot, B.",
  TITLE = 	"Fractals: {F}orm, {C}hance and {D}imension",
  YEAR = 	"1977",
  PUBLISHER = 	"Freeman, San Francisco"
}  

@Article{maris2007,
	AUTHOR = "Maris, E. and Schoffelen, J.-M. and Fries, P.",
	TITLE = "Nonparametric statistical testing of coherence differences",
	JOURNAL = "Journal of Neuroscience Methods",
	VOLUME = "163",
	NUMBER = "1",
	YEAR = "2007",
	PAGES = "161-175"
}

@Book{maste1995,
  AUTHOR = 	"Masters, T.",
  TITLE = 	"Neural, Novel \& Hybrid Algorithms for Time Series Prediction",
  YEAR = 	"1995",
  PUBLISHER = 	"John Willey \& Sons, Inc."}

@Book{melou2004,
  AUTHOR = 	"Meloun, M.and Militk\'{y}, J.",
  TITLE = 	"Statistick\'{a} anal\'{y}za experiment\'{a}ln\'{i}ch dat (Statistical analysis of experimental data , in czech)",
  PUBLISHER = 	"ACADEMIA",
  YEAR =	"2004"}  
  
@Article{meric1997,
    AUTHOR = 	"Merica, H. and Blois, R.",
    TITLE = 	"Relationship between the time courses of power in the frequency bands of human sleep {EEG}",
    YEAR = 	"1997",
    JOURNAL = 	"Neurophysiol Clin",
    VOLUME = 	"27",
    PAGES = 	"116-128"}

@Article{modde1989,
  author = "R. Moddemeijer",
  title = "On Estimation of Entropy and Mutual Information of Continuous Distributions",
  journal = "Signal Processing",
  volume = "16",
  number = "3",
  year = "1989",
  pages = "233-246",}


@Article{monge2014,
     author = {Monge-Alvarez, J},
     title =  {Higuchi Fractal Dimension - MatLab Function},
     journal = {\href{http://www.mathworks.com/matlabcentral/fileexchange/50290-higuchi-and-katz-fractal-dimension-measures}{http://www.mathworks.com/matlabcentral/fileexchange/50290-higuchi-and-katz-fractal-dimension-measures}},
    year = {2014},
%    crossref={http://www.mathworks.com/matlabcentral/fileexchange/50290-higuchi-and-katz-fractal-dimension-measures},
 }



@Book{morav1995,
  AUTHOR = 	"Mor\'{a}\v{n}, M.	",
  TITLE = 	"Praktick\'{a} elektroencefalografie",
  YEAR = 	"1995",
  PUBLISHER = 	"IDVPZ Brno	"}

@Article{morma2000,
AUTHOR = "Mormann, F. and Lehnertz, K. and David, P. and Elger, Ch. E.",
TITLE = "Mean phase coherence as a measure for phase synchronization and its application to the {EEG} of epilepsy patients",
JOURNAL = "Physica D",
VOLUME = "144", 
NUMBER = "3-4", 
YEAR = "2000",
PAGES = "358-369"
}



@Book{nevsi1997,
    AUTHOR = 	"Nev\v{s}\'{i}malov\'{a}, S. and others",
    TITLE = 	"Poruchy sp\'{a}nku a bd\v{e}n\'{i}",
    YEAR = 	"1997",
    PUBLISHER = 	"Maxdorf/Jessenius, Praha"}

@Article{nunez1997,
  AUTHOR = 	"Nunez, P. L. and Srinivasan, R. and Westdorp, A. F. and Wijesinghe, R. S. and Tucker, D. M. and Silberstein, R. B. and Cadusch, P. J.",
  TITLE =	"{EEG} coherency {I}: statistics, reference electrode, volume conduction, {L}aplacians, cortical imaging, and interpretation at multiple scales",
  JOURNAL =	"Electroencephalogr Clin Neurophysiol   ",
  VOLUME =	"103",
  NUMBER = "5",
  YEAR =	"1997",
  PAGES =	"499-515"}

@Article{ogilv1984,
  AUTHOR = 	"Ogilvie, R. D. and Wilkinson, R. T.",
  TITLE = 	"The detection of sleep onset: behavioral and physiological convergence",
  YEAR = 	"1984",
  JOURNAL = 	"Psychophysiology",
  VOLUME = 	"21",
  NUMBER = "5",
  PAGES = 	"510-520"}
  
@Article{ogilv1989,
  AUTHOR = 	"Ogilvie, R. D. and Wilkinson, R. T. and Allison, S.",
  TITLE = 	"The detection of sleep onset: behavioral, physiological, and subjective convergence",
  YEAR = 	"1989",
  JOURNAL = 	"Sleep",
  VOLUME = 	"12(5)",
  PAGES = 	"458-474"}
 
@Article{ogilv2001,
  AUTHOR = 	"Ogilvie, R. D.",
  TITLE = 	"The process of falling asleep",
  YEAR = 	"2001",
  JOURNAL = 	"Sleep Medicine Reviews",
  VOLUME = 	"5",
  NUMBER = "3",
  PAGES = 	"247-270"} 
  
@Article{olbri2003,
  AUTHOR = 	"Olbrich, E. and Achermann, P. and Meier, P. F.	",
  TITLE = 	"Dynamics of human sleep {EEG}",
  YEAR = 	"2003",
  JOURNAL = 	"Neurocomputing	",
  VOLUME = 	"52-54",
  PAGES = 	"857-862"}

@Article{orope1999,
   AUTHOR = 	"Oropesa, E. and Cycon, H. and Jobert, M.",
   TITLE = 	"Sleep stage classification using wavelet transform and neural network",
   YEAR = 	"1999",
   JOURNAL = 	"Technical Report",
   VOLUME = 	"8",
   PAGES = 	""}

@Article{osbor1989,
   AUTHOR = 	"Osborne, A. R. and Provenzale, A.",
   TITLE = 	"Finite correlation dimension for stochastic systems with power-law spectra",
   YEAR = 	"1989",
   JOURNAL = 	"Physica D",
   VOLUME = 	"35 (3)",
   PAGES = 	"357-381"}

@Article{palus1995,
	AUTHOR = "Palu\v{s}, M.",
	TITLE = "Testing for nonlinearity using redundancies: quantitative and qualitative aspects",
	JOURNAL = "Physica D",
	VOLUME = "80",
	NUMBER = "1-2",
	YEAR = "1995",
	PAGES = "186-205"
}
re
@Article{palus2005,
	AUTHOR = "Palu\v{s}, M. and Novotn\'{a}, D. and Tichavsk\'{y}, P.",
	TITLE = "Shifts of seasons at the European mid-latitudes: Natural fluctuations correlated with the North Atlantic Oscillation",	
	JOURNAL = "Geophys Res Lett",
	VOLUME = "32",
	NUMBER = "",
	YEAR = "2005",
	PAGES = "L12805"
}

%@article{palus2007,
%  title={Directionality of coupling from bivariate time series: How to avoid false causalities and missed connections},
%  author={Palu{\v{s}}, Milan and Vejmelka, Martin},
%  journal={Phys. Rev. E},
%  volume={75},
%  number={5},
%  pages={056211},
%  year={2007}
%}
%
%@article{palus2007b,
%  title={From nonlinearity to causality: statistical testing and inference of physical mechanisms underlying complex dynamics},
%  author={Palu{\v{s}}, Milan},
%  journal={Contemporary physics},
%  volume={48},
%  number={6},
%  pages={307--348},
%  year={2007},
%  publisher={Taylor \& Francis}
%}
%
%@article{vejme2008,
%  title={Inferring the directionality of coupling with conditional mutual information},
%  author={Vejmelka, Martin and Palu{\v{s}}, Milan},
%  journal={Physical Review E},
%  volume={77},
%  number={2},
%  pages={026214},
%  year={2008},
%  publisher={APS}
%} 
%
%@article{palus2014,
%  title={Cross-scale interactions and information transfer},
%  author={Palu{\v{s}}, Milan},
%  journal={Entropy},
%  volume={16},
%  number={10},
%  pages={5263--5289},
%  year={2014},
%  publisher={Multidisciplinary Digital Publishing Institute}
%}

@Article{parde1996,
   AUTHOR = "Pardey, J. and Roberts, S. and Tarassenko, L. and Stradling, J. ",
   TITLE = "A new approach to the analysis of the human sleep/wakefulness continuum",
   YEAR = "1996",
   JOURNAL = "Journal of Sleep Research",
   VOLUME = "5",
   NUMBER = "4",
   PAGES = "201-210"}

@Article{park2000,
   AUTHOR = "Park, H.-J. and Oh, J.-S. and Jeong, D.-U. and Park, K.-S.",
   TITLE = "Automated {S}leep {S}tage {S}coring {U}sing {H}ybrid {R}ule- and {C}ase-{B}ased {R}easoning",
   YEAR = "2000",
   JOURNAL = "Computers and Biomedical Research",
   VOLUME = "33",
   NUMBER = "5",
   PAGES = "330-349"}

@article{pecor1990,
  title={Synchronization in chaotic systems},
  author={Pecora, Louis M and Carroll, Thomas L},
  journal={Physical review letters},
  volume={64},
  number={8},
  pages={821},
  year={1990},
  publisher={APS}
}

@article{peng1994,
  title={Mosaic organization of DNA nucleotides},
  author={Peng, C-K and Buldyrev, Sergey V and Havlin, Shlomo and Simons, Michael and Stanley, H Eugene and Goldberger, Ary L},
  journal={Physical Review E},
  volume={49},
  number={2},
  pages={1685},
  year={1994},
  publisher={APS}
}

@Article{peng1995,
  AUTHOR = 	"Peng, C. and K. and Havlin, S. and Stanley, H. E. and Goldberger, A. L.",
  TITLE =	"Quantification of scaling exponents and crossover phenomena in nonstationary heartbeat time series",
  JOURNAL =	" Chaos",
  VOLUME =	"5",
  NUMBER = "1",
  YEAR =	"1995",
  PAGES =	"82-87"}

@Article{pered1998,
  AUTHOR = 	"Pereda, E. and Gamundi, A. and Rial, R. and Gonz{\'a}lez, J.",
  TITLE = 	"Nonlinear behaviour of human {EEG}: fractal exponent versus correlation dimension in awake and sleep stages",
  YEAR = 	"1998",
  JOURNAL = 	"Neurosci Lett",
  VOLUME = 	"250",
  NUMBER = "2",
  PAGES = 	"91-94"}

@Article{pered1999,
	AUTHOR = "Pereda, E. and Gamundi, A. and Nicolau, M. C. and Rial, R. and Gonz{\'a}lez, J.",
	TITLE = "Interhemispheric differences in awake and sleep human {EEG}: a comparison between non-linear and spectral measures",	
	JOURNAL = "Neurosci Lett",
	VOLUME = "263",
	NUMBER = "1",
	YEAR = "1999",
	PAGES = "37-40"
}

@Article{pered2001,
    AUTHOR = 	"Pereda, E. and others",
    TITLE = 	"Assessment of changing interdependencies between human electroencephalograms using           
    nonlinear methods",
    YEAR = 	"2001",
    JOURNAL = 	"Physica D",
    VOLUME = 	"148",
    PAGES = 	"147-158"}

@Article{pered2005,
	AUTHOR = "Pereda, E. and Quiroga, Q. R. and Bhattacharya, J.",
	TITLE = "Nonlinear multivariate analysis of neurophysiological signals",	
	JOURNAL = "Progress in Neurobiology",
	VOLUME = "77",
	NUMBER = "1-2",
	YEAR = "2005",
	PAGES = "1-37"
}

@Article{pezar1994,
    AUTHOR = 	"Pezard, L. and others",
    TITLE = 	"Non-linear forecasting measurements of multichannel {EEG} dynamics",
    YEAR = 	"1994",
    JOURNAL = 	"Electroencephalogr Clin Neurophysiol   ",
    VOLUME = 	"91",
    PAGES = 	"383-391"}

@INBOOK{plons2000,
	AUTHOR = "Plonsey, R.",
	EDITOR = "Bronzino, J. D.",	
	TITLE = "The Biomedical Engeneering Handbook",
	CHAPTER = "Volume Conductor Theory",
	PAGES = "9.1-9.8",
	PUBLISHER = "CRC Press",
	YEAR = "2000"
}

@Book{press1988,
    AUTHOR =	"Press, W. H. and others",
    TITLE =	"Numerical Recipes in C",
    YEAR =	"1988",
    PUBLISHER =	"Cambridge University Press",
    PAGES =	"398-470"}
    
@Article{princ1989,
   AUTHOR = 	"Principe, J. C. and Gala, S. K. and Chang, T. G.",
   TITLE = 	"Sleep staging automaton based on the theory of evidence",
   YEAR = 	"1989",
   JOURNAL = 	"IEEE Transactions on Biomedical Engineering",
   VOLUME = 	"36",
   NUMBER = "5",
   PAGES = 	"503-509"}
   
@Article{prinz1992,
   AUTHOR = 	"Prinz, P. N. and others",
   TITLE = 	"{EEG} markers of early Alzheimer's disease in computer selected tonic {REM} sleep",
   YEAR = 	"1992",
   JOURNAL = 	"Electroencephalogr Clin Neurophysiol   ",
   VOLUME = 	"83",
   PAGES = 	"36-43"}

@article{pyrag1996,
  title={Weak and strong synchronization of chaos},
  author={Pyragas, K},
  journal={Physical Review E},
  volume={54},
  number={5},
  pages={R4508},
  year={1996},
  publisher={APS}
}

@article{quiro2000,
  title = {Learning driver-response relationships from synchronization patterns},
  author = {Quiroga, R. Quian and Arnhold, J. and Grassberger, P.},
  journal = {Phys. Rev. E},
  volume = {61},
  issue = {5},
  pages = {5142--5148},
  year = {2000},
  month = {May},
  doi = {10.1103/PhysRevE.61.5142},
  url = {http://link.aps.org/doi/10.1103/PhysRevE.61.5142},
  publisher = {American Physical Society}
}

@Article{quiro2002,
	title = {Performance of different synchronization measures in real data: A case study on electroencephalographic signals},
	author = {Quian Quiroga, R.  and Kraskov, A.  and Kreuz, T.  and Grassberger, P. },
	journal = {Phys. Rev. E},
	volume = {65},
	number = {4},
	pages = {041903},
	year = {2002},
}

@INCOLLECTION{rappe2000,
	AUTHOR = "Rappelsberger, P.",
	EDITOR = "Bernd, S. and Krijzer, F. and Ferber, G. and Anderer, P.",	
	BOOKTITLE = "Electrophysiological Brain Research in Preclinical and Clinical Pharmacology and Related Fields",
	TITLE = "{EEG} coherence analysis: a method to visualise functional connections",
	PAGES = "33-44",
	PUBLISHER = "Facultas Universit?tsverlag, Wien (Austria)",
	YEAR = "2000"
}

@Book{recht1968,
  EDITOR = 	"Rechtschaffen, A. and Kales, A.",
  TITLE = 	"A Manual of Standardized Terminology, Techniques and Scoring System for Sleep Stages of Human Subject",
  YEAR = 	"1968",
  PUBLISHER = 	"US Government Printing Office, National Institute of Health Publication,                 Washington DC"}

@Inbook{recht2000,
    AUTHOR =	"Rechtschaffen, A. and Siegel, J. M.",
    CHAPTER =	"Sleep and Dreaming",
    EDITOR =	"Kandel, E. R. and Swartz, J. H. and Jessel, T. M.",
    TITLE =	"Principles of Neuroscience",
    YEAR =	"2000",
    PUBLISHER =	"McGraw-Hill, New York",
    PAGES = 	"936-947"}

@Article{richa1978,
  AUTHOR = 	"Richardson, G. S. and others",
  TITLE = 	"Excessive Daytime Sleepiness in Man: Multiple Sleep Latency Measurement in                   
  Narcoleptic and Control Subjects ",
  YEAR = 	"1978",
  JOURNAL = 	"Electroncephalogr. Clin. Neurophysiol.",
  VOLUME = 	"45",
  PAGES = 	"621-627"}
  
@Article{richt1993,
  AUTHOR = 	"Richter, M. and Schreiber, T.",
  TITLE = 	"Phase space embedding of electrocardiograms",
  YEAR = 	"1993",
  JOURNAL = 	"Phys Rev E",
  VOLUME = 	"58",
  PAGES = 	"1752-1763"}
    
@Article{rober1992,
    AUTHOR = 	"Roberts, S. and Tarassenko, L.",
    TITLE = 	"New method of automated sleep quantification",
    YEAR = 	"1992",
    JOURNAL = 	"Medical and Biological Engineering and Computing",
    VOLUME = 	"30",
    NUMBER = "5",
    PAGES = 	"509-517"}

@Article{roelf1997,
	AUTHOR = "Roelfsema, P. R. and Engel, A. K. and K{\"o}nig, P. and Singer, W.",
	TITLE = "Visuomotor integration is associated with zero time-lag synchronization among cortical areas",	
	JOURNAL = "Nature",
	VOLUME = "385",
	NUMBER = "",
	YEAR = "1997",
	PAGES = "157-161"
}

@article{roman2007,
  title={Estimation of the direction of the coupling by conditional probabilities of recurrence},
  author={Romano, M Carmen and Thiel, Marco and Kurths, J{\"u}rgen and Grebogi, Celso},
  journal={Physical Review E},
  volume={76},
  number={3},
  pages={036211},
  year={2007},
  publisher={APS}
}

@Article{rosa1999,
  AUTHOR = 	"Rosa, A. C. and Parrino, L. and Terzano, M. G.",
  TITLE = 	"Automatic detection of cyclic alternating pattern ({CAP}) sequences in sleep: preliminary results",
  YEAR = 	"1999",
  JOURNAL = 	"Clin Neurophysiol",
  VOLUME = 	"110",
  NUMBER = "4",
  PAGES = 	"585-592"}

@Article{rosch1993,
  AUTHOR = 	"R\H{o}schke, J. and Fell, J. and Beckmann, P.",
  TITLE = 	"The calculation of the first positive {L}yapunov exponent in sleep {EEG} data",
  YEAR = 	"1993",
  JOURNAL = 	"Electroencephalogr Clin Neurophysiol ",
  VOLUME = 	"86",
  NUMBER = "5",
  PAGES = 	"348-352"}

@Article{rosen1996,
	AUTHOR = "Rosenblum, M. G. and Pikovsky, A. S. and Kurths, J.",
	TITLE = "Phase Synchronization of Chaotic Oscillators",	
	JOURNAL = "Phys Rev Lett",
	VOLUME = "76",
	NUMBER = "11",
	YEAR = "1996",
	PAGES = "1804-1807"
}

@Book{rosip2001,
  AUTHOR = 	"R. Rosipal",
  TITLE = 	"Kernel-Based Regression and Objective Nonlinear Measures to Assess Brain Functionnig, PhD thesis",
  YEAR = 	"2001",
  PUBLISHER = 	"University of Paisley, Scotland",
  PAGES = 	""}

@Article{roth1999,
    AUTHOR = 	"Roth, C. and Achermann, P. and Borb\'{e}ly, A. A.",
    TITLE = 	"Frequency and state specific hemispheric asymmetries in the human sleep {EEG}",
    YEAR = 	"1999",
    JOURNAL = 	"Neurosci Lett",
    VOLUME = 	"271(3)",
    PAGES = 	"139-142"}

@article{rulko1995,
  title={Generalized synchronization of chaos in directionally coupled chaotic systems},
  author={Rulkov, Nikolai F and Sushchik, Mikhail M and Tsimring, Lev S and Abarbanel, Henry DI},
  journal={Physical Review E},
  volume={51},
  number={2},
  pages={980},
  year={1995},
  publisher={APS}
}

@Article{saast2007,
  AUTHOR = 	"Saastamoinen, A. and Huupponen,  E. and V{\"a}rri, A. and Hasan, J. and Himanen, S.-L.",
  TITLE =	"Systematic Performance evaluation of a continuos-scale sleep depth measure",
  JOURNAL =	"Medical Engineering \& Physics",
  VOLUME =	"29",
  NUMBER = "10",
  YEAR =	"2007",
  PAGES =	"1119-1131"}

@Article{sakai2003,
  AUTHOR = 	"Sakai, K. and Crochet, S.",
  TITLE = 	"A neural mechanism of sleep and wakefulness",
  YEAR = 	"2003",
  JOURNAL = 	"Sleep and Biological Rhythms",
  VOLUME = 	"1",
  PAGES = 	"29-42"}

@Article{santa1987,
  AUTHOR = 	"Santamaria, J. and Chiappa, KH.",
  TITLE = 	"The {EEG} of drowsiness in normal adults",
  YEAR = 	"1987",
  JOURNAL = 	"J Clin Neurophysiol",
  VOLUME = 	"4(4)",
  PAGES = 	"327-382"}

@Article{sauer1991,
    AUTHOR = 	"Sauer, T. and Yorke, J. A., and Casdagli, M.",
    TITLE = 	"Embedology",
    YEAR = 	"1991",
    JOURNAL = 	"Journal of Statistical Physics",
    VOLUME = 	"65",
    PAGES = 	"579-616"}

@Article{sauer1993,
    AUTHOR = 	"Sauer, T.",
    TITLE = 	"Time Series Prediction by Using Delay Coordinate Embedding",
    YEAR = 	"1993",
    JOURNAL = 	"In: Weigend, A. S. and Gershenfeld, N. A. and (Eds.):Time Series Prediction:               
    Forecasting the Future and Understanding the Past",
    PUBLISHER =	"Santa Fe Institute Studies in the Science of Complexity, Proc. Vol. XV,                    
    Addison-Wesley",
    PAGES = 	"175-193"}

@article{schep2002,
  title={Four methods to estimate the fractal dimension from self-affine signals},
  author={Schepers, Hans E and Van Beek, Johannes HGM and Bassingthwaighte, James B},
  journal={Engineering in Medicine and Biology Magazine, IEEE},
  volume={11},
  number={2},
  pages={57--64},
  year={2002},
  publisher={IEEE}
}
@article{schif1996,
  title={Detecting dynamical interdependence and generalized synchrony through mutual prediction in a neural ensemble},
  author={Schiff, Steven J and So, Paul and Chang, Taeun and Burke, Robert E and Sauer, Tim},
  journal={Physical Review E},
  volume={54},
  number={6},
  pages={6708},
  year={1996},
  publisher={APS}
}

@Article{schre1991,
    AUTHOR = 	"Schreiber, T. and Grassberger, P.",
    TITLE = 	"A simple noise reduction method for real data",
    YEAR = 	"1991",
    JOURNAL = 	"Physics Letters A",
    VOLUME = 	"160",
    PAGES = 	"411-418"}

@Article{schre1996,
    AUTHOR = 	"Schreiber, T. and Kaplan, D. T.",
    TITLE = 	"Nonlinear noise reduction for electrocardiograms",
    YEAR = 	"1996",
    JOURNAL = 	"Chaos",
    VOLUME = 	"6",
    PAGES = 	"87-92"}
       
@Article{schre2000,
    AUTHOR = 	"Schreiber, T. and Schmitz, A.",
    TITLE = 	"Surrogate time series",
    YEAR = 	"2000",
    JOURNAL = 	"Physica D",
    VOLUME = 	"142",
    PAGES = 	"346-382"}
%
%@article{schre2000b,
%  title={Measuring information transfer},
%  author={Schreiber, Thomas},
%  journal={Physical review letters},
%  volume={85},
%  number={2},
%  pages={461},
%  year={2000},
%  publisher={APS}
%}

@Article{shann1948,
	AUTHOR = "Shannon, C. E.",
	TITLE = "A Mathematical Theory of Communication",	
	JOURNAL = "Bell System Technical Journal",
	VOLUME = "27",
	NUMBER = "",
	YEAR = "1948",
	PAGES = "379-423"
}

@Article{shen2003,
    AUTHOR = 	"Shen, Y. and Olbrich, E. and Achermann, P. and Meier, P.F.",
    TITLE = 	"Dimensional complexity and spectral properties of the human sleep {EEG}",
    YEAR = 	"2003",
    JOURNAL = 	"Clin Neurophysiol",
    VOLUME = 	"114",
    NUMBER =  "2",
    PAGES = 	"199-209"}

%@misc{SIESTA,
%  note = 	"\textsc{WWW}. Siesta \textsc{URL}: http://www.ofai.at/research/nn/siesta/)"}
%%
%@Article{siget1995,
%  title = {Survival of deterministic dynamics in the presence of noise and the exponential decay of power spectra at high frequency},
%  author = {Sigeti, David E.},
%  journal = {Phys. Rev. E},
%  volume = {52},
%  number = {3},
%  pages = {2443--2457},
%  numpages = {14},
%  year = {1995},
%  month = {Sep},
%  doi = {10.1103/PhysRevE.52.2443},
%  publisher = {American Physical Society}
%}

@Article{shima2000,
    AUTHOR = 	"Shimada, T. and  Shiina, T. and  Saito, Y.",
    TITLE = 	"Detection of characteristic waves of sleep {EEG} by neural network analysis",
    YEAR = 	"2000",
    JOURNAL = 	"IEEE Transactions on Biomedical Engineering",
    VOLUME = 	"47 (3)",
    PAGES = 	"369-379"}

@Article{small2000,
    AUTHOR = 	"Small, M. and others",
    TITLE = 	"Nonlinear analysis of human {ECG} during sinus rhythm and arrhythmia",
    YEAR = 	"2000",
    JOURNAL = 	"Computers in Cardiology",
    VOLUME = 	" ",
    PAGES = 	"147-150"}

@Inproceedings{smith1986,
    AUTHOR = 	"Smith, J. R.",
    TITLE = 	"Automated analysis of sleep {EEG} data",
    YEAR = 	"1985",
    BOOKTITLE = "Handbook of {E}lectroencephalography and {C}linical {N}europhysiology",
    VOLUME = "3",
    PUBLISHER = "Elsevier, Amsterdam",
    PAGES = 	"131-147"}
    

@Article{smith1992,
    AUTHOR = 	"Smith, L. A.",
    TITLE = 	"Identification and prediction of low dimensional dynamics",
    YEAR = 	"1992",
    JOURNAL = 	"Physica D",
    VOLUME = 	"58",
    PAGES = 	"50-76"}

@Article{smith1993,
    AUTHOR = 	"Smith, L.",
    TITLE = 	"Does a Meeting in Santa Fe Imply Chaos?",
    YEAR = 	"1993",
    JOURNAL = 	"In: Weigend, A. S. and Gershenfeld, N. A. and (Eds.):Time Series Prediction:               
    Forecasting the Future and Understanding the Past",
    PUBLISHER =	"Santa Fe Institute Studies in the Science of Complexity, Proc. Vol. XV,                    
    Addison-Wesley",
    PAGES = 	"323-343"}

@Article{spenc2003,
  title = {Abnormal Neural Synchrony in Schizophrenia},
  author = {Spencer, K. M. and Nestor, P. G. and Niznikiewicz, M. A. and Salisbury, D. F. and Shenton, M. E. and McCarley, R. W.},
  journal = {J Neurosci},
  volume = {23},
  number = {19},
  pages = {7407 - 7411},
  year = {2003},
}
%
%@article{stam2002,
%  title={Synchronization likelihood: an unbiased measure of generalized synchronization in multivariate data sets},
%  author={Stam, CJ and Van Dijk, BW},
%  journal={Physica D: Nonlinear Phenomena},
%  volume={163},
%  number={3},
%  pages={236--251},
%  year={2002},
%  publisher={Elsevier}
%}
%  
@Article{stark1999,
    AUTHOR = 	"Stark, J.",
    TITLE = 	"Delay Embeddings for Forced Systems. I. Deterministic Forcing ",
    YEAR = 	"1999",
    JOURNAL = 	"Journal of Nonlinear Science",
    VOLUME = 	"9, Issue 3",
    PAGES = 	"255-332"}

@Article{steri1991,
	AUTHOR = "Steriade, M. and Dossi, R. C.  and Par\'{e}, D. and Oakson, D.",
	TITLE = "Fast oscillations (20 - 40 {H}z) in thalamocortical systems and their potentiation by mesopontine cholinergic nuclei in the cat",	
	JOURNAL = "Neurobiology",
	VOLUME = "88",
	NUMBER = "",
	YEAR = "1991",
	PAGES = "4396-4400"
}

@Article{steri1993,
	AUTHOR = "Steriade, M. and Nu\~{n}ez, A. and Amzica, F. ",
	TITLE = "A {N}ovel {S}low (<1 {H}z) {O}scillation of {N}eocortical {N}eurons in viva: {D}epolarizing and {H}yperpolarizing {C}omponents",	
	JOURNAL = "J Neurosci",
	VOLUME = "13",
	NUMBER = "8",
	YEAR = "1993",
	PAGES = "3252-3265"
}

@INCOLLECTION{steri1993b,
 author = "Steriade, M. ",
 title = "Cellular substrates of brain rhythms",
 booktitle = "Electroencephalography: Basic Principles, Clinical Applications and Related Fields",
 year  = "1993",
 editor = "Niedermeyer, E. and Lopes da Silva, F.",
 organization = " ",
 publisher = "Williams and Wilkins, Baltimore",
 pages = "27-62"}

@Article{steri1993c,
	AUTHOR = "Steriade, M. and McCormick, D. A. and Sejnowski, T. J. ",
	TITLE = "Talamocortical oscillations in the sleeping and aroused brain",	
	JOURNAL = "Science",
	VOLUME = "262",
	NUMBER = "",
	YEAR = "1993",
	PAGES = "679-685"
}

 @Article{stick1998,
    AUTHOR = 	"Stickgold, R.",
    TITLE = 	"Sleep: off-line memory reprocessing",
    YEAR = 	"1998",
    JOURNAL = 	"Trends in Cognitive Sciences	",
    VOLUME = 	"2",
    NUMBER = 	"12",
    PAGES = 	"484-492"}
    
@Article{stick2000,
    AUTHOR = 	"Stickgold, R. and James, L. T. and Hobson, J. A.",
    TITLE = 	"Visual discrimination learning requires sleep after training",
    YEAR = 	"2000",
    JOURNAL = 	"Nature Neuroscience",
    VOLUME = 	"3",
    PAGES = 	"1237-1238"}
%
%@article{sugih2012,
%  title={Detecting causality in complex ecosystems},
%  author={Sugihara, George and May, Robert and Ye, Hao and Hsieh, Chih-hao and Deyle, Ethan and Fogarty, Michael and Munch, Stephan},
%  journal={science},
%  volume={338},
%  number={6106},
%  pages={496--500},
%  year={2012},
%  publisher={American Association for the Advancement of Science}
%}

@Article{susma2005,
    AUTHOR = 	"\v{S}u\v{s}m\'{a}kov\'{a},  K.	",
    TITLE = 	"Complexity of {EEG} During Sleep Onset Process",
    YEAR = 	"2005",
    JOURNAL = 	"MEASUREMENT SCIENCE REVIEW",
    VOLUME = 	"",
    PAGES = 	""}

@Article{susma2008,
	AUTHOR = "\v{S}u\v{s}m\'{a}kov\'{a}, K. and Krakovsk\'{a}, A.",
	TITLE = "Discrimination ability of individual measures used in sleep stages classification",	
	JOURNAL = "Artificial Intelligence in Medicine",
	VOLUME = "44",
	NUMBER = "",
	YEAR = "2008",
	PAGES = "261-277"
}

@incollection{taken1981,
   AUTHOR = "Takens, F.",
   EDITOR = "Rand, D. A. and Young, L. S.",
   TITLE = 	"Detecting strange attractors in turbulence",
   BOOKTITLE = "Dynamical Systems and Turbulence",   		 
   YEAR = 	"1981",
   PUBLISHER = 	"Springer-Verlag, Berlin",
   PAGES = 	"366-381"}

@Article{tches2006,
	AUTHOR = "Tcheslavski, G.V.and Beex, A.A.",
	TITLE = "Phase synchrony and coherence analyses of {EEG} as tools to discriminate between children with and without attention deficit disorders",	
	JOURNAL = "Biomed Signal Process Contr",
	VOLUME = "1",
	NUMBER = "2",
	YEAR = "2006",
	PAGES = "151 - 161"
}

@Article{tepla2002,
   AUTHOR = 	"Teplan, M.",
   TITLE = 	"Fundamentals of {EEG} measurement",
   YEAR = 	"2002",
   JOURNAL = 	"Measurement Science Review",
   VOLUME = 	"2",
   PAGES = 	"1-11"}
%   
%@article{tepla2006,
%  title={EEG responses to long-term audio--visual stimulation},
%  author={Teplan, M and Krakovsk{\'a}, A and {\v{S}}tolc, S},
%  journal={International Journal of Psychophysiology},
%  volume={59},
%  number={2},
%  pages={81--90},
%  year={2006},
%  publisher={Elsevier}
%}
    
@Article{terza1985,
  AUTHOR = 	"Terzano, M. G. and Mancia, D. and Salati,  M. R. and Costani, G.and Decembrino, A. and Parrino L.",
  TITLE = 	"The cyclic alternating pattern as a physiologic component of normal {NREM} sleep",
  YEAR = 	"1985",
  JOURNAL = 	"Sleep",
  VOLUME = 	"8",
  NUMBER = "2",
  PAGES = 	"137-145"}
 
@Article{terza1988,
  AUTHOR = 	"Terzano, M. G. and Parrino, L. and Spaggiari, M. C",
  TITLE = 	"The cyclic alternating pattern sequences in the dynamic organisation of sleep",
  YEAR = 	"1988",
  JOURNAL = 	"Electroencephalogr Clin Neurophysiol   ",
  VOLUME = 	"69",
  PAGES = 	"437-447"
}

@Article{terza2001,
  AUTHOR = 	"Terzano, M. G. and others",
  TITLE = 	"Altas, rules, and recording techniques for the scoring of cyclic alternating pattern ({CAP})   in human sleep",
  YEAR = 	"2001",
  JOURNAL = 	"Sleep Medicine	",
  VOLUME = 	"2",
  PAGES = 	"537-553"
}

@Article{thatc2005,
  AUTHOR = 	"Thatcher, R. W. and North, D. and Biver, C.",
  TITLE =	"{EEG} and intelligence: {R}elations between {EEG} coherence, {EEG} phase delay and power",
  JOURNAL =	"Clin Neurophysiol",
  VOLUME =	"116",
  NUMBER = "9",
  YEAR =	"2005",
  PAGES =	"2129-2141"}

@Article{theil1986,
    AUTHOR = "Theiler, J.",
    TITLE = "Spurious dimension from correlation algorithms applied to limited time-series data",
    YEAR = "1986",
    JOURNAL = "Phys. Rev. A",
    VOLUME = "34",
    PAGES = "2427-2432"
}

@Article{theil1992,
  AUTHOR = "Theiler, J. and Eubank, S. and Longtin, A. and Galdrikian, B. and Farmer, J. D.",
  TITLE = "Testing for nonlinearity in time series: the method of surrogate data",
  YEAR = "1992",
  JOURNAL = "Physica D",
  VOLUME = "58",
  NUMBER = "1-4",
  PAGES = "77-94"
}

@Article{theil1996,
  AUTHOR = "Theiler, J. and Rapp, P. E.",
  TITLE = "Re-examination of the evidence for low-dimensional, nonlinear structure in the human electroencephalogram",
  YEAR = "1996",
  JOURNAL = "Electroencephalogr Clin Neurophysiol   ",
  VOLUME = "98",
  PAGES = "213-222"
}

@Book{therr1989,
  AUTHOR = 	"Therrien, C.",
  TITLE = 	"Decision, Estimation and Classification: An Introduction to Pattern Recognition and Related Topics",
  YEAR = 	"1989",
  PUBLISHER = 	"Wiley, New York"}

@Article{vande2005,
  AUTHOR = "van den Berg, J. and others",
  TITLE = "Electroencephalography and subjective ratings of sleep deprivation",
  YEAR = "2005",
  JOURNAL = "Sleep Medicine",
  VOLUME = "6",
  PAGES = "231?240"}

@Article{velaz2005,
	AUTHOR = "Perez Velazquez, J. L.",
	TITLE = "Brain, behaviour and mathematics: Are we using the right approaches?",	
	JOURNAL = "Physica D",
	VOLUME = "212",
	NUMBER = "",
	YEAR = "2005",
	PAGES = "161?182"
}

%@article{Vlach2010,
%  title=''Nonuniform state-space reconstruction and coupling detection'',
%  author=''Vlachos, Ioannis and Kugiumtzis, Dimitris'',
%  journal=''Physical Review E'',
%  volume=''82'',
%  number=''1'',
%  pages=''016207'',
%  year=''2010'',
%  publisher=''APS''
%}
%  
@INPROCEEDINGS{vogel2001,
  AUTHOR = "Vogel, F. and Holm, S. and Lingj{\ae}rde, O. C.",
  TITLE = "Spectral moments and time domain representation of photoacoustic signals used for detection of crude oil in produced water",
  BOOKTITLE =	"Proc. Nordic Symp. on Physical Acoustics",
  YEAR = "2001",
  ADDRESS =	"Ustaoset, Norway"}

@Article{watte2004,
  AUTHOR = "Watters, P. A. and Martin, F.",
  TITLE = "A method for estimating long-range power law correlations from the electroencephalogram",
  YEAR = "2004",
  JOURNAL = "Biological Psychology",
  VOLUME = "66",
  NUMBER = "1",
  PAGES = "79-89"}

@Book{weige1993,
  AUTHOR = "Weigend, A. S. and Gershenfeld, N. A. and (Eds.)	",
  TITLE = "{Time {S}eries {P}rediction: {F}orecasting the {F}uture and {U}nderstanding the {P}ast}	",
  YEAR = "1993",
  PUBLISHER = "Santa Fe Institute Studies in the Science of Complexity, Proc. Vol. XV, Addison-Wesley"}

@Article{weiss1973,
	AUTHOR = "Weiss, M. S.",
	TITLE = "Non-Gaussian properties of the {EEG} during sleep",	
	JOURNAL = "Electroencephalogr Clin Neurophysiol ",
	VOLUME = "34",
	NUMBER = "2",
	YEAR = "1973",
	PAGES = "200-202"
}

@Article{welch1967,
	AUTHOR = "Welch, P.D.",
	TITLE = "The {U}se of {F}ast {F}ourier {T}ransform for the {E}stimation of {P}ower {S}pectra: {A} {M}ethod {B}ased on {T}ime {A}veraging {O}ver {S}hort, {M}odified {P}eriodograms",	
	JOURNAL = "IEEE Trans. Audio Electroacoustics",
	VOLUME = "AU-15 ",
	NUMBER = "",
	YEAR = "1967",
	PAGES = "70-73"
}
  
@Article{werth1997,
  AUTHOR = "Werth, E. and Achermann, P. and Dijk, D. J. and Borb{\'e}ly, A. A.",
  TITLE = "Spindle frequency activity in the sleep {EEG}: individual differences and topographic distribution",
  YEAR = "1997",
  JOURNAL = "Electroencephalogr Clin Neurophysiol   ",
  VOLUME = "103",
  NUMBER = "5",
  PAGES = "535-542"}

@Article{white98,
  AUTHOR = "White, D. P. and Gibb, T. J.",
  TITLE = "Evaluation of a computerized polysomnographic system",
  YEAR = "1998",
  JOURNAL = "Sleep",
  VOLUME = "21",
  NUMBER = "2",
  PAGES = "188-196"}
   
@Article{wrigh1995,
  AUTHOR = "Wright, K. P. Jr and Badia, P. and Wauquier, A.",
  TITLE = "Topographical and temporal patterns of brain activity during the transition from wakefulness to sleep",
  YEAR = "1995",
  JOURNAL = "Sleep",
  VOLUME = "18(10)",
  PAGES = "880-889"}

@misc{wwwLDA,
  URL = "http://www.stat.psu.edu/~jiali/"
 }
  
@Article{zeitl1997,
  AUTHOR = "Zeitlhofer, J. and others",
  TITLE = "Topographic distribution of sleep spindles in young healthy subjects",
  YEAR = "1997",
  JOURNAL = "Journal of Sleep Research",
  VOLUME = "6(3)",
  PAGES = "149-155"} 
   
@Article{zoube2007,
  AUTHOR = 	"Zoubek, L. and Charbonnier, S. and Lesecq, S. and Buguet, A. and Chapotot, F.",
  TITLE =	"Feature selection for sleep/wake stages classification using data driven methods",
  JOURNAL =	"Biomed Signal Process Contr",
  VOLUME =	"2",
  NUMBER = "3",
  YEAR =	"2007",
  PAGES =	"171-179"}
 































